Natural Language Commanding via Program Synthesis

We present Semantic Interpreter, a natural language-friendly AI system for productivity software such as Microsoft Office that leverages large language models (LLMs) to execute user intent across application features. While LLMs are excellent at understanding user intent expressed as natural language, they are not sufficient for fulfilling application-specific user intent that requires more than text-to-text transformations. We therefore introduce the Office Domain Specific Language (ODSL), a concise, high-level language specialized for performing actions in and interacting with entities in Office applications. Semantic Interpreter leverages an Analysis-Retrieval prompt construction method with LLMs for program synthesis, translating natural language user utterances to ODSL programs that can be transpiled to application APIs and then executed. We focus our discussion primarily on a research exploration for Microsoft PowerPoint.

==> tables/results.tex <==
\begin{table}[t!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccccccc@{}}
\toprule
\makecell[t]{Entity \\ Classifier} & \makecell[t]{Requires Context \\ Classifier} & \makecell[t]{Code \\ Correction} & \makecell[c]{$k$} & \makecell[t]{Exact} & \makecell[t]{Normalized} & \makecell[t]{Subprogram \\ Exact} & \makecell[t]{Subprogram \\ Normalized} & \makecell[t]{Manual Check \\ Valid} & \makecell[t]{None} & \makecell[t]{Error} & \makecell[t]{Pass Rate \\ (\%)} \\
\midrule
\cmark & \cmark & \cmark & 0 & 0 & 10 & 0 & 1 & 8 & 28 & 150 & 9.64 \\
 \cmark & \cmark & \cmark & 1 & 20 & 89 & 5 & 40 & 20 & 13 & 10 & 88.32 \\
 \cmark & \cmark & \cmark & 3 & 28 & 91 & 8 & 39 & 19 & 6 & 6 & 93.91 \\
 \midrule
 \cmark & \cmark & \cmark & 5 & 37 & 96 & 9 & 37 & 12 & 1 & 5 & \textbf{96.95} \\
 \midrule
  \cmark & \cmark & \cmark & 7 & 32 & 92 & 10 & 32 & 21 & 1 & 9 & 94.92 \\
  \cmark & \cmark & \cmark & 9 & 26 & 66 & 8 & 40 & 24 & 4 & 29 & 83.25 \\
  \xmark & \cmark & \cmark & 5 & 17 & 89 & 8 & 38 & 16 & 15 & 14 & 85.23 \\
  \cmark & \xmark & \cmark & 5 & 21 & 69 & 5 & 42 & 18 & 34 & 8 & 78.68 \\
  \xmark & \xmark & \cmark & 5 & 14 & 75 & 5 & 49 & 15 & 28 & 11 & 80.20 \\
  \cmark & \cmark & \xmark & 5 & 33 & 93 & 8 & 36 & 11 & 1 & 15 & 91.88 \\
  \bottomrule

\end{tabular}%
}
\vspace{1mm}
\caption{Results of ablation study, running the evaluation procedure discussed in Section~\ref{sec:eval} on variants of \system.}
\label{table:results}
\end{table}
